Constraints on Inner Disk Evolution Timescales: A Disk Census of the eta Chamaeleontis Young Cluster

We present new L' (3.8-micron) observations of stars in the nearby (~97 pc) young (~6 Myr) compact cluster around eta Chamaeleontis, obtained with the European Southern Observatory's Very Large Telescope in Paranal, Chile. Our data, combined with J,H, Ks photometry from the 2-Micron All Sky Survey, reveal that only two of the 12 members surveyed harbor L'-band excesses consistent with optically thick inner disks; both are also likely accretors. Intriguingly, two other stars with possible evidence for on-going accretion, albeit at very low rates, do not show significant infrared excess: this may imply substantial grain growth and/or partial clearing of the inner disk region, as expected in planet formation scenarios. Our findings suggest that eta Cha stars are in an epoch when disks are rapidly evolving, perhaps due to processes related to planet building, and provide further constraints on inner disk lifetimes.

==> figurelist.tex <==
\clearpage
\plotone{f1.eps}
\clearpage
\plotone{f2.eps}
\clearpage
\plotone{f3a.eps}
\clearpage
\plotone{f3b.eps}
\clearpage

